The Communication Complexity of Set Intersection and Multiple Equality Testing

In this paper we explore fundamental problems in randomized communication complexity such as computing Set Intersection on sets of size $k$ and Equality Testing between vectors of length $k$. Sa\u{g}lam and Tardos and Brody et al. showed that for these types of problems, one can achieve optimal communication volume of $O(k)$ bits, with a randomized protocol that takes $O(\log^* k)$ rounds. Aside from rounds and communication volume, there is a \emph{third} parameter of interest, namely the \emph{error probability} $p_{\mathrm{err}}$. It is straightforward to show that protocols for Set Intersection or Equality Testing need to send $\Omega(k + \log p_{\mathrm{err}}^{-1})$ bits. Is it possible to simultaneously achieve optimality in all three parameters, namely $O(k + \log p_{\mathrm{err}}^{-1})$ communication and $O(\log^* k)$ rounds? In this paper we prove that there is no universally optimal algorithm, and complement the existing round-communication tradeoffs with a new tradeoff between rounds, communication, and probability of error. In particular: 1. Any protocol for solving Multiple Equality Testing in $r$ rounds with failure probability $2^{-E}$ has communication volume $\Omega(Ek^{1/r})$. 2. There exists a protocol for solving Multiple Equality Testing in $r + \log^*(k/E)$ rounds with $O(k + rEk^{1/r})$ communication, thereby essentially matching our lower bound and that of Sa\u{g}lam and Tardos. Our original motivation for considering $p_{\mathrm{err}}$ as an independent parameter came from the problem of enumerating triangles in distributed ($\textsf{CONGEST}$) networks having maximum degree $\Delta$. We prove that this problem can be solved in $O(\Delta/\log n + \log\log \Delta)$ time with high probability $1-1/\operatorname{poly}(n)$.

==> 2-round.tex <==
\section{Lower bound on two-round randomized protocol} \label{sect:lb}

\begin{theorem} \label{thm:2-round}
\begin{enumerate}
\item Any two-round randomized protocol $Q$ for $\EQ^k$ that has failure probability less than $2^{-k}$ has complexity $\Omega(k^{1.5})$. 
\item Any two-round deterministic protocol $Q$ for $\EQ^k$ that errors on at most a $2^{-k}$ fraction of all possible inputs has complexity at least $\Omega(k^{1.5})$.
\end{enumerate}
\end{theorem}

Consider any deterministic protocol $Q$, we draw the input of Alice and Bob independently from a uniform distribution on $[t]^k$. Let $X = (X_1, X_2, \ldots, X_k)$ and $Y = (Y_1, Y_2, \ldots, Y_k)$ be the random variable denoting Alice's and Bob's input, and $M_1$ and $M_2$ be the random variable denoting the message sent in the first and the second round. Without loss of generality, we assume these messages all have the same fixed length $c_1 = c'k^{1.5}$ for some constant $c' \geq 0$ that we will determine later. Notice that $M_1$ partitions the universe $[t]^k$ into $2^{c_1}$ sets. For a given $M_1 = m_1 \in \{0, 1\}^{c_1}$, we use $S_{m_1}$ to denote the set of input $x \in [t]^k$ such that the corresponding first message is $m_1$. We omit the subscript $m_1$ when the first message is fixed from context. 

We sample the input for Alice in a two-stage manner: First, Alice samples her message $M_1$ with the following distribution $\mu$ on $\{0, 1\}^{c_1}$ where $\mu(m) = |S_m|/2^{c_1}$. Then she will sample a uniformly random element $X$ in $S_m$. Notice that the marginal distribution for $X$ is still uniform. We overload the notation $\mu$ to also denote the uniform distribution on $[t]^k$.

The following fact is elementary in communication complexity and information theory. 

\begin{fact}\label{fac:entropy}
\[
H(M_1) \leq c'k^{1.5}
\]
Therefore, 
\[
I(X;M_1) \leq H(M_1) \leq c'k^{1.5}
\]
\end{fact}

The mutual information $I(X ; M_1) = H(X) - H(X \mid M_1)$ measures how much information about $X$ we learn because of $M_1$ \emph{on average}. For the purpose of our argument, we also define the information gain about $X$ for a specific message $m_1$, which is $I(X ; M_1=m_1) = H(X) - H(X \mid M_1=m_1)$.

\begin{lemma}\label{lem:small-info}
\begin{enumerate}
\item There exists a set of messages $\M$ with $\mu(\M) \ge 1/2$ such that for all message $m_1 \in \M$, the information gained on $X$ satisfies $I(X ; M_1 = m_1) \le 2c'k^{1.5}$.
\item For each message $m_1 \in \M$, there exists a set of coordinates $\I'_{m_1}\subseteq [k]$ of size $|\I'_{m_1}| = k/3$  such that for all coordinate $i \in \I'_{m_1}$, the information gained on $X_i$ satisfies $I(X_i ; M_1 = m_1) \le 4c'\sqrt{k} - 1$.
\end{enumerate}
\end{lemma}
\begin{proof}
We first prove the first statement. From Fact~\ref{fac:entropy}, we have
\begin{align*}
    I(X; M_1) = \sum_{m_1 \in \{0, 1\}^{c_1}} \mu(m_1)I(X; M_1 = m_1) \leq c'k^{1.5}
\end{align*}
Suppose for all set of messages $\M$ such that $\mu(\M) \geq 1/2$, we have $I(X; M_1 = m_1) > 2c'k^{1.5}$ for all $m_1 \in \M$, then $I(X; M) \geq \sum_{m_1 \in \M} \mu(m_1) I(X; M_1 = m_1) > c'k^{1.5}$, which is a contradiction.

As to the second statement, for each message $m_1 \in \M$, we have
\begin{align*}
\sum_{i=1}^k I(X_i ; M_1 = m_1)
& = \sum_{i=1}^k H(X_i) - \sum_{i=1}^k H(X_i \mid M_1=m_1) \\
& \le H(X) - H(X \mid M_1=m_1) \\
& = 2c'k^{1.5},
\end{align*}
where the second step comes from the independence of $X_i$ and the simple fact that the joint entropy is no more than the sum of individual entropies.

Suppose for contradiction that there are no more than $k/3$ coordinates $i$ satisfying $I(X_i ; M_1 = m_1) \le 4c'\sqrt{k} - 1$. The summation over remaining coordinates of individual information gain will be at least $2k/3 \cdot (4c'\sqrt{k}-1) > 2c'k^{1.5}$ for $k$ large enough, contradicting the first statement.
\end{proof}

Now we argue that for a large set of coordinates where Bob learns little about Alice's input, Bob will have no choice but to send his entire input on these coordinates to Alice. By choosing her message $M_1$ to be $m_1$, Alice commits her input to the set $S = S_{m_1}$. As Bob samples his input $Y$ uniformly randomly from $[t]^k$, say $y = (y_1, y_2, \ldots, y_k)$, from his perspective, given a coordinate $i \in [k]$, since Alice has yet to commit her input to any particular element in $S$, the probability that $X_i = y_i$ is either $0$ when $S$ does not contain any vector whose $i$-th coordinate is $y_i$, or some positive number which is the fraction of vectors in $S$ whose $i$-th coordinate is $y_i$. We argue that when the information gain from $m_1$ is not much greater than its average value, this probability is large for a significant fraction of values $y_i$. This is formalized in the following lemma:


\begin{lemma}\label{lem:high-prob}
For each message $m_1 \in \M$ and each coordinate $i \in \I'_{m_1}$, there exists at least a $2^{-4c'\sqrt{k}}$ fraction of $y_i \in [t]$ such that
\begin{equation}\label{eqn:col}
\Pr[X_i = y_i \mid M_1 = m_1] \ge 2^{-(c+o(1))k}.
\end{equation}
\end{lemma}
\begin{proof}
We prove this lemma via contradiction, where the $o(1)$ term in the exponent is fixed to be $k^{-1/2}$ \footnote{In fact, it can be anything at least $\omega(\log k/k)$.}. 
We show that if no more than $2^{-4c'\sqrt{k}}$ fraction of $y_i \in [t]$ satisfies \eqref{eqn:col}, then the maximum possible entropy $H(X|M_1 = m_1)$ will is too small, which contradicts the second statement of Lemma~\ref{lem:small-info}. 
Fix an index $i \in \I_{m_1}'$, define $p_u$ to be the probability that $X_i = u$,
\[
p_u\coloneqq \Pr[X_i=u \mid M_1=m_1].
\]
Clearly, these probabilities sum up to 1:
\[
\sum_{u=1}^{t}p_u=1.
\]
Now we denote $U_1$ to be the set of all $u$'s such that $p_u\ge 2^{-(c+k^{-1/2})k}$, and $U_0=[k] \setminus U_1$ to be the rest. 
Since by our assumption $|U_1|\le 2^{-4c'\sqrt{k}}\cdot t$, by concavity of the entropy function, the maximum entropy is obtained when we have all $p_u$'s with $u \in U_0$ reach $p_{U_0}=2^{-(c+k^{-1/2})k}$, then divide the remaining probability evenly among $U_1$.
Hence $p_u$ for all $u\in U_1$ is:
\[
p_{U_1}=\frac{1-|U_0|\cdot 2^{-(c+k^{-1/2})k}}{|U_1|}
\]
Hence, the maximum entropy we can obtain is:
\begin{align*}
H(X_i \mid m_1)  &= -\sum_{u=1}^t p_u\log p_u \\
            &= -\sum_{u\in U_0}p_u\log p_u-\sum_{v\in U_1}p_v\log p_v \\
            &= -|U_0|\cdot p_{U_0}\log p_{U_0}-|U_1|\cdot p_{U_1}\log p_{U_1}.
\end{align*}
We first bound the first term,
\begin{align*}
-|U_0|\cdot p_{U_0}\log p_{U_0} &\le t\cdot2^{-(c+k^{-1/2})k}(c+k^{-1/2})k \\
                                &= 2^{-\sqrt{k}}(c+k^{-1/2})k \\
                                &= o(1).
\end{align*}
For the second term, notice that
\begin{align*}
-|U_1|\cdot p_{U_1}\log p_{U_1} &\le -\log p_{U_1} \\
                                &=|U_1|-\log\left(1-|U_0| \cdot 2^{-(c+k^{-1/2})k}\right) \\
                                &\le ck-4c'\sqrt{k}+o(1).
\end{align*}
Therefore, combining these two terms, we have
\[
H(X_i \mid m_1) \le ck-4c'\sqrt{k}+o(1).
\]
By Lemma~\ref{lem:small-info}, we have $I(X_i \mid m_1) = H(X_i) - H(X_i \mid m_1) \leq 4c'\sqrt{k} - 1$, thus $H(X_i \mid m_1) \geq ck - 4c'\sqrt{k} + 1$, the bound above leads to a contradiction when $k$ is large enough.
\end{proof}

\begin{lemma} \label{lem:large-set-large-prob}
For each message $m_1 \in \M$, there exists a set of coordinates $\I_{m_1} \subseteq \I'_{m_1}$ of size $|\I_{m_1}| = \sqrt{k}/(8c')$ and at least a $2^{-k/2}$ fraction of $y \in [t]^k$ such that \eqref{eqn:col} holds for all coordinate $i \in \I_{m_1}$.
\end{lemma}
\begin{proof}
In fact, we can pick an arbitrary subset $\I_{m_1} \subseteq \I'_{m_1}$ of size $|\I_{m_1}| = \sqrt{k}/(8c') < k/3$. For each coordinate $i \in \I_{m_1}$, by Lemma~\ref{lem:high-prob}, there exists a subset $\Y_{i,m_1} \subseteq [t]$ of size $|\Y_{i,m_1}| = t/2^{4c'\sqrt{k}}$ such that \eqref{eqn:col} holds for all $y_i \in \Y_{i,m_1}$.

Let $\Y_{m_1}$ be the set of vector $y$'s such that $y_i \in \Y_{i,m_1}$ for all $i \in \I_{m_1}$. Clearly, this set accounts for a $(2^{-4c'\sqrt{k}})^{\sqrt{k}/(8c')} = 2^{-k/2}$ fraction of $y \in [t]^k$. This concludes the proof of the lemma.
\end{proof}

Now we can prove Theorem~\ref{thm:2-round}.

\begin{proof}
The final finishing step for this argument is to argue that to achieve an error probability of $2^{-k}$, Bob will have no choice but to send his entire input for every coordinate in $\I_{m_1}$ back to Alice, thus resulting in  an $\Omega(k^{1.5})$ lower bound for the protocol. \\
Suppose for the purpose of contradiction that Bob's message back to Alice is of size $c'k^{1.5}$. Now from Lemma~\ref{lem:large-set-large-prob}, we know that there are $2^{-k/2}\cdot 2^{ck^2}$ possible inputs for Bob where \eqref{eqn:col} holds for at least $\sqrt{k}/(8c')$ coordinates, we call these inputs bad.
\xnote{The original argument is actually flawed. We are still considering how to prove this part.}
Combining this with Lemma~\ref{lem:small-info}, we can conclude that at least a $1/2\cdot 2^{-k/2}\geq 2^{-k}$ fraction of all possible inputs will err, if the communication complexity is $O(k^{1.5})$. \\
Therefore, we conclude that any two-round deterministic protocol $Q$ for $EQ_k$ that errs on at most $2^{-k}$ fraction of all possible inputs has complexity at least $\Omega(k^{1.5})$.
\end{proof}



==> new-alg.tex <==
\subsection{new-alg}

\begin{itemize}
    \item Error budget: $E' = 3E$.
    \item Communication budget: $3\alpha_jEk^{1/r}$ for round $j$ with $\alpha_1 = \alpha_2 = 1$.
    \item First round: $k_0 = k, l_1^* = l_1 = 3\alpha_1Ek^{1/r-1}$.
    \item Round $j \ge 2$:
        \begin{itemize}
            \item $k_{j-1} = E' / l_{j-1}^*, l_j = 3\alpha_jEk^{1/r} / k_{j-1} = \alpha_jk^{1/r}l_{j-1}^*$.
            \item Conduct $\log r$ parallel tests with $k_{j-1}^{(i)} = 2^{-(i-1)}k_{j-1}, l_j^{(i)} = 2^{i-1}l_j/i^c$ for the $i$th one, where $0 < c < 1$. (A parallel test with $k_{j-1}^{(i)} < 1$ is equivalent to a hash test.)
            \item Total volume $\sum_i k_{j-1}^{(i)} l_j^{(i)} = k_{j-1}l_j \sum_i i^{-c} = 3\alpha_jEk^{1/r} \cdot O(\log^{1-c} r)$.
            \item Let $0 \le i_j^* < \log r$ be the smallest $i$ such that the $(i+1)$st parallel test fails; set $i_j^* = \log r$ if all parallel tests succeed.
            \item If $i_j^* = 0$, terminate as $k_{j-1}^{(1)}l_{j-1}^* = E'$; if $1 \le i_j^* < \log r$, the error budget has been exhausted by a fraction of $\beta_{j-1} = k_{j-1}^{(i_j^*+1)}l_{j-1}^* / E'= 2^{-i_j^*}$; if $i_j^* = \log r$, set $\beta_{j-1} = 1/r$.
            \item Since the $i_j^*$th parallel test succeeds, each remaining coordinate gets $l_j^* = 2^{i_j^*-1}l_j/(i_j^*)^c = l_j/(2\beta_{j-1}\log^c(1/\beta_{j-1}))$ valid bits.
            \item Set $\alpha_{j+1} = 2\beta_{j-1}\log^c(1/\beta_{j-1})$, ensuring that $l_j = k^{1/r}l_{j-1} = 3Ek^{j/r-1}$.
        \end{itemize}
    \item Total volume:
        \begin{itemize}
            \item Logarithmic terms are always dominated.
            \item By definition of $i_j^*$, $\sum_j \beta_j \le 2$.
            \item Because of the concavity of $x\log^c(1/x)$ on $[0,1]$ for $0 < c < 1$, $\sum_j \alpha_j = 2 + \sum_j 2\beta_j\log^c(1/\beta_j)$ reaches its maximum $O(\log^c r)$ when all $\beta_j$'s are equal.
            \item Overall communication is bounded by $3Ek^{1/r} \cdot O(\log^{1-c} r) \cdot \sum_j \alpha_j = O(Ek^{1/r}\log r)$.
        \end{itemize}
\end{itemize}

==> recycle_bin.tex <==

\begin{theorem}

\end{theorem}

\paragraph{Outline}
We want to prove that an $r$-rounds deterministic protocol for $k$-equality that has distributional error $2^{-E}$ uses at least $\Omega(E k^{1/r}/r)$ bits. We do the following:

\paragraph{A Sampling Experiment}

Fixed a deterministic protocol $Q$, we want to analyze the error probability of $Q$ under the uniform distribution. 
To analyze this probability, we first describe a sampling process of How Alice and Bob sample their respective inputs. 
The sampling process is as follows:
Let $\D_{-1}$ and $\D_0$ be the uniform distribution on $[t]^k$ that corresponds to Alice's and Bob's input. And $I_0 = [k]$ to be the set of all coordinates. 
Since the first message $m_1$ from Alice is a function of Alice's input, and $\D_{-1}$ induces a distribution on Alice's first message. 
Alice can first sample her first message $m_1$ according to this distribution and send it to Bob. 
This commits Alice's input $x$ to a subset $S_1 \subseteq [t]^n$. 
Let $\D_1$ be the distribution of Alice's input conditioned on the first message $m_1$.
By definition, $\D_1$ is a uniform distribution on $S_1$.

Upon receiving $m_1$, Bob can identify a subset of coordinates $I_1$ where Alice did not reveal much information on.
Then instead of sampling from $\D_0$, Bob change his input distribution to another distribution $\D_{1}'$ which is identical to $\D_1$ on the set of coordinates $I_1$, 
and conditioned on the input on $I_1$, the rest of the coordinates are sampled according to the distribution $\D_0$ conditioned on the input on $I_1$. Here, $\D_1'$ is identical to $\D_1$ on $I_1$, and uniform on $I_0 \setminus I_1$.
$\D_1'$ induces a distribution on Bob's message $m_2$. Bob samples his message and send it to Alice. 
This commits Bob's input to a set $S_2$ and and we use $\D_2$ to denote Bob's input distribution conditioned on the message $m_1, m_2$.

At the end of round $2$, Alice receives $m_2$, find a the set of coordinate $I_2$ corresponds to $m_2$ and further modify her input distribution in a similar manner to obtain a new input distribution $\D_2'$: 
$\D_2'$ is identical to $\D_2$ on the coordinates of $I_2$ and conditioned on these coordinate, the distribution on rest of the coordinate is identical to the conditional distribution of $\D_1$.

This process continues until the last round. Suppose the last message is sent from Alice to Bob, 
Bob will then be left with a set of exactly one coordinate $I_r = \{i_r\}$ where there is still too much entropy left on Alice input. 
He generates his input distribution $\D_r'$ for the last round to be the same as Alice's distribution $\D_r$ on the index set $I_r$, and conditioned on the assignment on $I_r$, the distribution is the same as $\D_{r-1}$ on the rest of the coordinate conditioned in $I_r$.

\paragraph{Notation}
Suppose in the $j$-th round, Alice sends her message $m_j$ to Bob:


\begin{enumerate2}
\item[$\D_{j-1}$] Bob's input distribution given all messages up until $m_{j-1}$.
\item[$\hD_{j-1}$] Alice's input distribution after all her modifications, \emph{before} sending her message $m_j$.
\item[$\D_j$] Alice's input distribution that she commits to \emph{after} sending her message $m_j$.
\item[$\tD_{j}$] Bob's distribution given all messages until $m_{j-1}$ and after chopping off low probability points.
More specifically, we first project $\D_{j-1}$ onto the coordinate $I_j$, then we remove any point $y$ with probability less than $1/2 t^{-|I_j|}$. Conditioned on we avoiding these points on the projection, the resultant distribution is $\tD_{j}$ 
\item[$I_j$] TBD.
\item[$\bD_{j}$] We will show that a large fraction (measured according to $D_j$) of points on $I_j$ satisfy the following bounded ratio property: 
\[
\Pr_{\D_{j} \mid I_j}(y) / \Pr_{\tD_j \mid I_j}(y) \leq 2^{E/(10r)}
\]
Conditioned on we hitting these ``good'' points on distribution $\D_j$, the distribution is $\bD_j$.
\item[$\hD_j$] The input distribution on all coordinates obtained by first copying the distribution $\bD_j$ on $I_j$, then condition on any assignment on $I_j$, we follow the conditional distribution on the rest of the coordinates according to $\D_{j-1}$.
\end{enumerate2}

\xnote{New Definitions}
\begin{enumerate2}
\item[$\D_{j-1}$] Bob's input distribution, \emph{before} Alice sends her message $m_j$.
\item[$\hD_{j-1}$] Alice's input distribution after her various modifications, \emph{before} sending her message $m_j$.
\item[$\D_j$] Alice's input distribution that she commits to, \emph{after} sending her message $m_j$.
\item[$\tD_{j}$] Bob's first modification, performed on his original input distribution $\D_{j-1}$.
Specifically, Bob removes any points $y\in\D_{j-1}$ whose probability when projected onto $I_j$ is less than $2^{-|I_j|}t^{-|I_j|}$:
\[
\Pr_{\D_{j-1} \mid I_j}(y_{\mid I_j})\leq 2^{-|I_j|}t^{-|I_j|}
\]
We denote the resulting distribution $\tD_{j}$.
\item[$I_j$] From $I_j$, we can find a subset $I_j\subset I_{j-1}$ with size $k^{1-j/r}$ that will leak little information on coordinates $I_j$(a more rigorous definition will be provided later).
\item[$\bD_{j}$] Bob's second modification, performed on Alice's new distribution $\D_j$.
We will show that there exists a set of points on $I_j$ with large probability mass on $\D_j$, satisfying the following property:
\[
\Pr_{\D_{j} \mid I_j}(y) / \Pr_{\tD_j \mid I_j}(y) \leq 2^{E/(10r)}
\]
We denote the distribution of $\D_{j}$ restricted to the support of this set of points as $\bD_{j}$.
\item[$\hD_{j}$] Bob's final modification to his input. He first copies the distribution of $\bD_{j}$ on the coordinate set $I_j$, and then for any specific assignment inside this set, he follows the conditional distribution of $\D_{j-1}$ on the rest of the coordinates $I_0 / I_j$.
\end{enumerate2}



\begin{lemma}\label{lem:entropy-reduction-message}
For each round $1 \le j \le r$, there exists a set of messages $\M_j$ of probability mass at least $\mu(\M_j) \ge 3/4$, such that
\[
H(\hD_{j-1 \mid \I_{j-1}}) - H(\D_{j \mid \I_{j-1}}) \le 4c'Ek^{1/r}/r
\]
holds for every message $m_j \in \M_j$.
\end{lemma}
\begin{proof}
Suppose for contradiction that there exists more than one fourth of messages $m_j$ satisfying
\[
H(\hD_{j-1 \mid \I_{j-1}}) - H(\D_{j \mid \I_{j-1}}) > 4c'Ek^{1/r}/r.
\]
The expected information gain from $M_j$ will then exceed the message size $|M_j| = c'Ek^{1/r}/r$, which is impossible for sure.
\end{proof}

\jnote{The constants need to be tweaked later.}
\begin{lemma}\label{lem:entropy-reduction-index}
For each round $1 \le j \le r$ and each message $m_j \in \M_j$, if $\I_{j-1}$ satisfies that
\[
H(\hD_{j-1 \mid \J}) \ge \left(cE - 100c'E^{(j-1)/r}/r\right) |\J|
\]
holds for every nonempty subset $\J \subseteq \I_{j-1}$, then there exists a subset $\I'_j \subseteq \I_{j-1}$ of size $|\I'_j| = |\I_{j-1}|/2$ such that
\[
H(\hD_{j-1 \mid \J}) - H(\D_{j \mid \J}) \le 10c'E^{j/r}|\J|/r,
\]
and consequently
\[
H(\D_{j \mid \J}) \ge \left(cE - 20c'E^{j/r}/r\right) |\J|
\]
holds for every nonempty subset $\J \subseteq \I'_j$, provided that $E^{1/r}$ is large enough.
\end{lemma}
\begin{proof}
Suppose $\J_1,\J_2,\ldots,\J_u$ are disjoint subsets of $\I_{j-1}$, each of which satisfies
\[
H(\hD_{j-1 \mid \J}) - H(\D_{j \mid \J}) > 10c'E^{j/r}|\J|/r,
\]
while none of subsets of $\J_0 = \I_{j-1} \setminus (\bigcup_{v=1}^u \J_v)$ does. By assumption, we have
\begin{align*}
H(\hD_{j-1 \mid (\I_{j-1} \setminus \J_0)}) - H(\D_{j \mid (\I_{j-1} \setminus \J_0)}) \ge {} & H(\hD_{j-1 \mid (\I_{j-1} \setminus \J_0)}) - \sum_{v=1}^u H(\D_{j \mid \J_v}) \\
\ge {} & \left(cE - 100c'E^{(j-1)/r}/r\right) |\I_{j-1} \setminus \J_0| \\
+ {} & \sum_{v=1}^u \left(10c'E^{j/r}|\J_v|/r - H(\hD_{j-1 \mid \J_v})\right) \\
\ge {} & 10c' |\I_{j-1} \setminus \J_0| \left(E^{j/r} - 10E^{(j-1)/r}\right)/r \\
\ge {} & 8c' E^{j/r}|\I_{j-1} \setminus \J_0|/r
\end{align*}
when $E^{1/r}$ is large enough. On the other hand, by Lemma~\ref{lem:entropy-reduction-message}, we also know
\[
H(\hD_{j-1 \mid (\I_{j-1} \setminus \J_0)}) - H(\D_{j \mid (\I_{j-1} \setminus \J_0)}) \le H(\hD_{j-1 \mid \I_{j-1}}) - H(\D_{j \mid \I_{j-1}}) \le 4c'E^{j/r}|\I_{j-1}|/r,
\]
which implies $|\I_{j-1} \setminus \J_0| \le |\I_{j-1}|/2$. Therefore, picking an arbitrary subset $\I'_j \subseteq \J_0$ of size $|\I'_j| = |\I_{j-1}|/2$ concludes the proof.
\end{proof}

\begin{lemma}\label{lem:low-prob-point}
Given any distribution $D$ defined over $U$. Let $V \subseteq U$ be the subset of values $x \in U$ such that $D(x) \le f/|U|$, where $0 < f < 1$. Then, the total probability mass over $V$ is at most $f$.
\end{lemma}
\begin{proof}
This is quite straightforward since $\sum_{x \in V} D(x) \le f/|U| \cdot |U| = f$.
\end{proof}

\begin{lemma}\label{lem:ratio-bound}
Given any two distributions $p$ and $q$ both defined over $U$ of size $2^E$ such that
\begin{enumerate2}
\item $\supp(q) \subseteq \supp(p)$;
\item $H(q) \ge E - I$, where $I = o(E)$;
\item $p(x) \ge 2^{-E-I}$ holds for every value $x \in \supp(p)$.
\end{enumerate2}
Then, there exists a subset of values $V \subseteq \supp(q)$ such that
\begin{enumerate2}
\item the total probability mass over $V$ measured by $q$ is at least $1/2$;
\item for each value $x \in V$, $q(x)/p(x) \le 2^{4I}$.
\end{enumerate2}
\end{lemma}
\begin{proof}
Let $W$ be the set of values $x \in \supp(q)$ such that $q(x) / p(x) > 2^{4I}$, which also implies $q(x) > 2^{-E+3I}$. Suppose for contradiction that the total probability mass over $W$ measured by $q$ is at least $f > 1/2$. Then, the entropy of $q$ is at most
\begin{align*}
    H(q) & \leq \sum_{x \in W} q(x) \log q(x)^{-1} + \sum_{x \in (V \setminus W)} q(x) \log q(x)^{-1} \\
         & \leq f (E - 3I) + (1-f) \log \frac{2^E}{1-f} \\
         & \leq E - 3I/2 - (1-f)\log(1-f),
\end{align*}
which clearly contradicts $H(q) \ge E - I$ when $I$ is large enough.
\end{proof}

\begin{lemma}\label{lem:large-intersection}
For each round $1\leq j \leq r$, there exists a set of messages $\M'_j$ with probability mass at least $\mu(\M'_j)\geq 1/2$, such that for every $m_j\in\M'_j$, the probability nmass of $\supp(\D_{j\mid I_j}) \cap \supp(\tD_{j\mid I_j})$ on $\D_{j\mid I_j}$ is at least $1/2$.
\end{lemma}
\begin{proof}
We present a proof by contradiction. Throughout the proof, we will always consider distributions as if they were projected onto $I_j$.

From Lemma~\ref{lem:entropy-reduction-message} and Lemma~\ref{lem:entropy-reduction-index}, we can find set $\I'_{j}$ and still keep $\mu(\M_j)\geq 3/4$ of all messages. We show that for at least $\mu(\M'_j)\geq 1/2$ total mass of messages, this lemma holds. Now if this is not true, then we can find a set of messages $\overline{\M}_j$ with probability mass at least $\mu(\overline{\M}_j)\geq3/4-1/2=1/4$, such that for every $m_j\in\overline{\M}_j$, and for every possible subset $\I_j\subseteq\I'_{j}$ with $|\I_j|=k^{1-j/r}$, the mass of $\supp(\D_j) \cap \supp(\tD_j)$ on $\D_j$ is no more than $1/2$. This means that
\[
\sum_{\substack{y\in\supp(\D_j) \\ y\in\supp(\D_{j-1}) \\ y\notin\supp(\tD_{j})}} \Pr_{\D_j}(y)\geq \frac12.
\]
Now consider the following quantity:
\[
Z = \sum_{\substack{\forall m_j \\ \forall \I_j\subseteq \I_{j-1},|\I_j|=k^{1-j/r} \\ y\in\supp(\D_{j-1}) \\ y\notin\supp(\tD_{j})}} \Pr_{\D_j}(y)\cdot\mu(m_j).
\]
First, we can lower bound $Z$, by observing the fact that for $1/4$ of the messages, and any choice of $\I_j\in\I'_j$, $\sum D_j(y_j)\geq 1/2$. Therefore, we have
\[
Z\geq \frac14\cdot\binom{1/2|\I_{j-1}|}{|\I_j|}\cdot\frac12.
\]
Next, we can also upper bound $Z$. Now notice that when we take the weighted average of all distributions $D_j$ for different messages $m_j$, we are essentially calculating $\hD_{j-1}$. However, since we enumerated all different subsets $\I_j\subseteq\I_{j-1}$, every point in $\hD_{j-1}$ is counted exactly $\binom{|\I_{j-1}|}{|\I_{j}|}$ times. We will later prove that $|\hD_{j-1}|/|D_{j-1}|$ for all $j$ is constant.

We already know the total probability mass of points $y$ in $\D_{j-1}$ satisfying $y\in\supp(\D_{j-1})$ and $y\notin\supp(\tD_{j})$ to be bounded by $2^{-|\I_j|}t^{-|I_j|}$.
Therefore we can also upper bound Z:
\[
Z\leq \binom{|\I_{j-1}|}{|\I_{j}|}\cdot 2^{-|\I_j|}t^{-|I_j|}\cdot O(1).
\]
Combing the lower bound and the upper bound, we can result in contradiction:
\[
\binom{|\I_{j-1}|}{|\I_{j}|}\cdot 2^{-|\I_j|}t^{-|I_j|}\cdot O(1) < \frac14\cdot\binom{1/2|\I_{j-1}|}{|\I_j|}\cdot\frac12.
\]
\end{proof}



\begin{fact}[Chain rule for KL divergence]\label{fac:kl-divergence}
Let $k > 1 $ and let $p(x_1, x_2, \ldots, x_k)$ and $q(y_1, y_2, \ldots, y_k)$ be two probability distributions on $k$-dimensional vectors with $\supp(p) \subseteq \supp(q)$. Suppose $p_i(x_i)$ and $q_i(y_i)$ are its respective marginal distribution on the $i$-th coordinate. Then
\[
\kl{p}{q} \geq \sum_{i = 1}^k \kl{p_i}{q_i}
\]
\end{fact}


\begin{lemma}\label{lem:good-message}
Given any discrete distribution $\A$, and a set of messages $\M$ each with length $N$.
Denote the random variable defined on $\A$ to be $X$, and a message $m=m(x)\in\M$ is assigned to every $x\in\supp(\A)$.

Define the random variable $M$ on $\M$ to be
\[
\Pr[M=m_1]=\sum_{m(x)=m_1}\Pr[X=x].
\]

Further define the probability of a set of messages $\M_1\subseteq\M$ to be
\[
\Pr[M\in\M_1]=\sum_{m(x)\in\M_1}\Pr[X=x].
\]

There exists a set of messages $\M_0$ with probability at least $1/3$, such that the following conditions hold for every $m_0\in\M_0$:
\begin{align*}
\h{X}-\h{X\mid M=m_0} &\le 3N \\
\kl{X\mid M=m_0}{X} &\le 3N.
\end{align*}
\end{lemma}

\begin{proof}
We can bound entropy loss and mutual information as follows,
\[
\h{X}-\h{X\mid M} = \I(X;M) \leq H(M) \leq \log|\M| \leq N,
\]
where the last inequality follows because there are at most $2^N$ different messages with length $N$. 

By writing out $\h{X}-\h{X\mid M}$ explicitly, we have
\[
\sum_{m}\Pr[M=m]\cdot(\h{X}-\h{X\mid M=m})\leq N.
\]

Therefore, by Markov's inequality, the set $\M'$ of all messages $m'$ satisfying $\h{X}-\h{X\mid M=m'}>3N$ has probability no greater than $1/3$.

We can also write out $\I(X;M)$ explicitly to obtain
\begin{align*}
N&\geq I(X;M) \\
&= \sum_{x,m}\Pr[X=x \land M=m]\log\frac{\Pr[X=x \land M=m]}{\Pr[X=x]\Pr[M=m]} \\
&= \sum_{m}\Pr[M=m]\sum_{x}\Pr[X=x \mid M=m]\log\frac{\Pr[X=x\mid M=m]}{\Pr[X=x]} \\
&= \sum_{m}\Pr[M=m]\kl{X\mid M=m}{X}.
\end{align*}

$\left(A\mid B\;\|\;C\right)$ vs $\left(A\mid B\;\middle\|\;C\right)$

Therefore, similarly by Markov's Inequality, the set $\M''$ of all messages $m''$ satisfying $\kl{X\mid M=m''}{X}>3N$ has probability no greater than $1/3$.

We now pick $\M_0=\M\setminus(\M'\cup\M'')$, then for every message $m_0\in\M_0$, both conditions will hold. In addition, the probability of $\M_0$ is at least $1-1/3-1/3=1/3$.
\end{proof}


We now prove a ``Markov style'' inequality that relates the KL divergence, which can be interpreted as the average log distortion of getting from one probability distribution to another distribution, 
\begin{lemma} \label{lem:div-to-ratio}
Let $p(x)$ and $q(x)$ be discrete distributions such that $\supp(p) \subseteq \supp(q)$, then for any $0 < \alpha < 1$,
\[
\Pr_{x\sim p}\left[\frac{p(x)}{q(x)} \geq 2^{(\kl{p}{q} + 1)/\alpha}\right] < \alpha
\]
\end{lemma}
\begin{proof}
Let $\X_0 = \left\{ x \in \supp(p) \mid p(x) / q(x) \geq 2^{(\kl{p}{q} + 1)/\alpha}\right\}$ and $\X_1 = \supp(p) \setminus \X_0$. For contradiction assume $p(\X_0) = \alpha_0 > \alpha$. Then the contribution of $\X_0$ to the KL divergence is at least:
\[
\sum_{x \in \X_0} p(x) \log \frac{p(x)}{q(x)} \geq \alpha_0 \cdot \frac{\kl{p}{q} + 1}{\alpha} > \kl{p}{q} + 1
\] 
Now we want to bound the (negative) contribution of the remaining elements, define $p'$ on $\X_1$ to be $p'(x) = p(x) / (1 - \alpha_0)$. By definition of $\alpha_0$, $p'$ is a distribution on $\X_1$.
\begin{align*}
     &\sum_{x \in \X_1} p(x) \log \frac{p(x)}{q(x)} \\
    =& (1 - \alpha_0)\sum_{x \in \X_1} p'(x) \log \frac{p(x)}{q(x)} \\
    =& -(1 - \alpha_0)\sum_{x \in \X_1} \frac{p(x)}{1 - \alpha_0} \log \frac{q(x)}{p(x)} \\
    \geq& -(1 - \alpha_0) \log \sum_{x \in \X_1} \frac{p(x)}{1 - \alpha_0} \frac{q(x)}{p(x)} \\
    =& -(1 - \alpha_0) \log \frac{q(\X_1)}{1 - \alpha_0} \\
    \geq& (1 - \alpha_0) \log (1 - \alpha_0) \\
    \geq& -1 \tag{}
\end{align*}
Here, the first inequality is by the convexity of $-\log$ function. And the last inequality is because $(1-x)\log(1 - x) \geq -1$ on its domain. 
Hence the overall KL divergence is more than $\kl{p}{q}$, giving a contradiction.
\end{proof}


A useful property of KL divergence is the chain rule. 
\begin{proposition}
Let $X$ and $Y$ be two random variables and $p$, $q$ be two distributions on $x$ and $y$, then
\begin{equation}
    \kl{p(x, y)}{q(x, y)} = \kl{p(x)}{q(x)} + \kl{p(y \mid x)}{q(y \mid x)} 
\end{equation}
\end{proposition}

Here, $\kl{p(y \mid x)}{q(y \mid x)} = \sum_{x} p(x) \sum_{x} p(x\mid y)\log p(x\mid y)/q(x\mid y)$ is called conditional divergence. An immediate corollary of this is that the KL divergence of two joint distributions are no less than sum of the KL divergence of their marginals. 

\begin{corollary}
Let $p(x_1, x_2, \ldots, x_k)$ and $q(x_1, x_2, \ldots, x_k)$ be two distributions on $k$-dimensional vectors such that $\supp(p) \subseteq \supp(q)$. and let $p(x_i)$ and $q(x_i)$ are their respective marginals on the $i$-th coordinates, then 
\[
\kl{p}{q} \geq \sum_i \kl{p_i}{q_i}
\]
\end{corollary}
\begin{proof}
We show the inequality for two variables $x$ and $y$, and the general case for $k$ variables follows from induction
\begin{align*}
    \kl{p(x, y)}{q{x, y}} &= \kl{p(x)}{q(x)} + \kl{p(y \mid x)}{q(y \mid x)} \\
                          &= \kl{p(x)}{q(x)} + \sum_{x} p(x) \sum_{x} p(x\mid y)\log p(x\mid y)/q(x\mid y) \\
                          &\geq \kl{p(x)}{q(x)} + \sum_{x} p(x) 
\end{align*}
\end{proof}

\xnote{New Proof}
\begin{proof}
We show the inequality for two variables $X$ and $Y$, and then the general case for $k$ variables follows from induction.
\begin{align*}
    \kl{p(x, y)}{q{x, y}} &= \kl{p(x)}{q(x)} + \kl{p(y \mid x)}{q(y \mid x)} \\
                          &= \kl{p(x)}{q(x)} + \sum_{x} p(x) \sum_{x} p(y\mid x)\log \frac{p(y\mid x)}{q(y\mid x)}
\end{align*}

Consider the following multivariate function $f(p, q)=p\log\frac pq$. Clearly\xnote{needs actual proof} this is a convex.

Now for every $x\in\supp(X)$ and $y\in\supp(Y)$, we define point $Z_{x, y}=(p(y\mid x), q(y\mid x))$.

By the multivariate Jensen's inequality, for every fixed $y$ we have
\begin{align*}
f(\sum_{x} p(x)Z_{x, y}) &\leq \sum_{x}p(x)f(Z_{x,y}) \\
(\sum_{x}p(x)p(y\mid x))\log \frac{\sum_{x}p(x)p(y\mid x)}{q(y\mid x)} &\leq \sum_{x}p(x)\p(y\mid x)\log \frac{p(y\mid x)}{q(y\mid x)} \\
p(y)\log \frac{p(y)}{q(y)} &\leq \sum_{x}p(x)\p(y\mid x)\log \frac{p(y\mid x)}{q(y\mid x)}
\end{align*}
\end{proof}



\begin{lemma}\label{lem:hash-test}
Suppose that Alice and Bob needs to perform $L$ hash equality tests on each of $N$ coordinates, and the total number of coordinates that are actually different can be bounded by $K$. If $\log(N/K)=o(L)$, this test can be done within $O(KL)$ bits of communication.
\end{lemma}
\begin{proof}
Let Alice and Bob draw $L$-bit universal hashing factions for each of the $N$ coordinates, and compute their binary strings. Denote Alice's output for the $i$-th output to be $x_i$, and Bob's $i$-th output to be $y_i$. For coordinates where Alice and Bob agree, their hash must be the same. Therefore, we can bound the block Hamming distance of $x=(x_1,\ldots,x_N)$ and $y=(y_1,\ldots,y_N)$ to be $BH-dist(x, y)\leq K$. by Lemma~\ref{lem:block-hamming-distance}, Alice and Bob can communicate their strings using $O(KL+K\log(N/K))=O(KL)$ bits.
\end{proof}
